Galactic Orbital Effects on Pulsar Timing

In the currently accepted paradigm, dark matter is hypothesized as an explanation of the flat rotation curves of galaxies under the assumption of virialized orbits. The use of millisecond pulsar timing as a probe of Galactic dark matter content is explored as a means of relaxing this assumption. A method of inference of the Galactic potential using the frequency derivative $\dot{\nu}$ is produced, and an estimate for a virialized Galactic rotation curve is given through direct observation of acceleration. The data set used includes 210 pulsars with known $\dot{\nu}$ and astrometric properties, a subset of which also have measured $\ddot{\nu}$. In principle, this enables the exploration of kinematic effects, but in practice, $\ddot{\nu}$ values are found to be too imprecise at present to adequately constrain radial velocities of pulsars. Additionally, surface magnetic field strengths are inferred from $\dot{\nu}$ and the magnetic spin-down contribution to $\ddot{\nu}$ is estimated. For several pulsars the radial velocity is known, and the kinematic contribution to $\ddot{\nu}$ is estimated accordingly. The binary orbital periods of PSR J1713+0747 and other binary pulsars are also used to constrain Galactic mass density models.

==> bibliography.tex <==
\bibliographystyle{unsrt}
\begin{singlespace}
\bibliography{bibliography}
\end{singlespace}
